Reinforcement Learning based Autonomous Multi-Rotor Landing on Moving Platforms

Multi-rotor UAVs suffer from a restricted range and flight duration due to limited battery capacity. Autonomous landing on a 2D moving platform offers the possibility to replenish batteries and offload data, thus increasing the utility of the vehicle. Classical approaches rely on accurate, complex and difficult-to-derive models of the vehicle and the environment. Reinforcement learning (RL) provides an attractive alternative due to its ability to learn a suitable control policy exclusively from data during a training procedure. However, current methods require several hours to train, have limited success rates and depend on hyperparameters that need to be tuned by trial-and-error. We address all these issues in this work. First, we decompose the landing procedure into a sequence of simpler, but similar learning tasks. This is enabled by applying two instances of the same RL based controller trained for 1D motion for controlling the multi-rotor's movement in both the longitudinal and the lateral directions. Second, we introduce a powerful state space discretization technique that is based on i) kinematic modeling of the moving platform to derive information about the state space topology and ii) structuring the training as a sequential curriculum using transfer learning. Third, we leverage the kinematics model of the moving platform to also derive interpretable hyperparameters for the training process that ensure sufficient maneuverability of the multi-rotor vehicle. The training is performed using the tabular RL method Double Q-Learning. Through extensive simulations we show that the presented method significantly increases the rate of successful landings, while requiring less training time compared to other deep RL approaches. Finally, we deploy and demonstrate our algorithm on real hardware. For all evaluation scenarios we provide statistics on the agent's performance.

==> bibliography.tex <==
\begin{thebibliography}{10}
\providecommand{\url}[1]{#1}
\csname url@samestyle\endcsname
\providecommand{\newblock}{\relax}
\providecommand{\bibinfo}[2]{#2}
\providecommand{\BIBentrySTDinterwordspacing}{\spaceskip=0pt\relax}
\providecommand{\BIBentryALTinterwordstretchfactor}{4}
\providecommand{\BIBentryALTinterwordspacing}{\spaceskip=\fontdimen2\font plus
\BIBentryALTinterwordstretchfactor\fontdimen3\font minus
  \fontdimen4\font\relax}
\providecommand{\BIBforeignlanguage}[2]{{%
\expandafter\ifx\csname l@#1\endcsname\relax
\typeout{** WARNING: IEEEtran.bst: No hyphenation pattern has been}%
\typeout{** loaded for the language `#1'. Using the pattern for}%
\typeout{** the default language instead.}%
\else
\language=\csname l@#1\endcsname
\fi
#2}}
\providecommand{\BIBdecl}{\relax}
\BIBdecl

\bibitem{Rodriguez-Ramos2019}
A.~Rodriguez-Ramos, C.~Sampedro, H.~Bavle, P.~de~la Puente, and P.~Campoy, ``A
  deep reinforcement learning strategy for uav autonomous landing on a moving
  platform,'' \emph{Journal of Intelligent \& Robotic Systems}, vol.~93, no.~1,
  pp. 351--366, 2019.

\bibitem{Mo2018}
H.~Mo and G.~Farid, ``Nonlinear and adaptive intelligent control techniques for
  quadrotor uav – a survey,'' \emph{Asian Journal of Control}, vol.~21,
  no.~2, pp. 989--1008, 2019.

\bibitem{Sutton2015}
R.~S. Sutton and A.~G. Barto, \emph{Reinforcement Learning: An Introduction
  Second edition, in progress}.\hskip 1em plus 0.5em minus 0.4em\relax
  Cambridge, Massachusetts; London, England: The MIT Press, 2015.

\bibitem{Mnih2013}
V.~Mnih, K.~Kavukcuoglu, D.~Silver, A.~Graves, I.~Antonoglou, D.~Wierstra, and
  M.~Riedmiller, ``{Playing Atari with Deep Reinforcement Learning},'' 2013.

\bibitem{Hasselt2010}
H.~Hasselt, ``Double q-learning,'' in \emph{Advances in Neural Information
  Processing Systems}, J.~Lafferty, C.~Williams, J.~Shawe-Taylor, R.~Zemel, and
  A.~Culotta, Eds., vol.~23.\hskip 1em plus 0.5em minus 0.4em\relax Curran
  Associates, Inc., 2010.

\bibitem{Lampton2009}
A.~Lampton and J.~Valasek, ``Multiresolution state-space discretization method
  for q-learning,'' in \emph{2009 American Control Conference}, 2009, pp.
  1646--1651.

\bibitem{Wang2016}
P.~Wang, Z.~Man, Z.~Cao, J.~Zheng, and Y.~Zhao, ``Dynamics modelling and linear
  control of quadcopter,'' in \emph{2016 International Conference on Advanced
  Mechatronic Systems (ICAMechS)}, 2016, pp. 498--503.

\bibitem{Wenzel2011}
K.~E. Wenzel, A.~Masselli, and A.~Zell, ``Automatic take off, tracking and
  landing of a miniature uav on a moving carrier vehicle,'' \emph{Journal of
  Intelligent \& Robotic Systems}, vol.~61, no.~1, pp. 221--238, 2011.

\bibitem{Araar2017}
O.~Araar, N.~Aouf, and I.~Vitanov, ``Vision based autonomous landing of
  multirotor uav on moving platform,'' \emph{Journal of Intelligent \& Robotic
  Systems}, vol.~85, no.~2, pp. 369--384, 2017.

\bibitem{Hu2015}
B.~Hu, L.~Lu, and S.~Mishra, ``Fast, safe and precise landing of a quadrotor on
  an oscillating platform,'' in \emph{2015 American Control Conference (ACC)},
  2015, pp. 3836--3841.

\bibitem{Ling2014}
K.~Ling, D.~Chow, A.~Das, and S.~L. Waslander, ``Autonomous maritime landings
  for low-cost vtol aerial vehicles,'' in \emph{2014 Canadian Conference on
  Computer and Robot Vision}, 2014, pp. 32--39.

\bibitem{Gautam2015}
A.~Gautam, P.~Sujit, and S.~Saripalli, ``Application of guidance laws to
  quadrotor landing,'' in \emph{2015 International Conference on Unmanned
  Aircraft Systems (ICUAS)}, 2015, pp. 372--379.

\bibitem{Vlantis2015}
P.~Vlantis, P.~Marantos, C.~P. Bechlioulis, and K.~J. Kyriakopoulos,
  ``Quadrotor landing on an inclined platform of a moving ground vehicle,''
  \emph{Proceedings - IEEE International Conference on Robotics and
  Automation}, vol. 2015-June, pp. 2202--2207, 2015.

\bibitem{Borowczyk2017}
A.~Borowczyk, D.-T. Nguyen, A.~{Phu-Van Nguyen}, D.~Q. Nguyen, D.~Saussié, and
  J.~L. Ny, ``Autonomous landing of a multirotor micro air vehicle on a high
  velocity ground vehicle,'' \emph{IFAC-PapersOnLine}, vol.~50, no.~1, pp.
  10\,488--10\,494, 2017, 20th IFAC World Congress.

\bibitem{Falanga2017}
D.~Falanga, A.~Zanchettin, A.~Simovic, J.~Delmerico, and D.~Scaramuzza,
  ``Vision-based autonomous quadrotor landing on a moving platform,'' in
  \emph{2017 IEEE International Symposium on Safety, Security and Rescue
  Robotics (SSRR)}, 2017, pp. 200--207.

\bibitem{Zhong2016}
D.~Zhong, X.~Zhang, H.~Sun, Z.~Ren, and J.~Han, ``A vision-based auxiliary
  system of multirotor unmanned aerial vehicles for autonomous rendezvous and
  docking,'' in \emph{2016 International Joint Conference on Neural Networks
  (IJCNN)}, 2016, pp. 4586--4592.

\bibitem{Miyazaki2018}
R.~Miyazaki, R.~Jiang, H.~Paul, K.~Ono, and K.~Shimonomura, ``Airborne docking
  for multi-rotor aerial manipulations,'' in \emph{2018 IEEE/RSJ International
  Conference on Intelligent Robots and Systems (IROS)}, 2018, pp. 4708--4714.

\bibitem{Kooi2021}
J.~E. Kooi and R.~Babuška, ``Inclined quadrotor landing using deep
  reinforcement learning,'' in \emph{2021 IEEE/RSJ International Conference on
  Intelligent Robots and Systems (IROS)}, 2021, pp. 2361--2368.

\bibitem{Shi2019}
G.~Shi, X.~Shi, M.~O’Connell, R.~Yu, K.~Azizzadenesheli, A.~Anandkumar,
  Y.~Yue, and S.-J. Chung, ``Neural lander: Stable drone landing control using
  learned dynamics,'' in \emph{2019 International Conference on Robotics and
  Automation (ICRA)}, 2019, pp. 9784--9790.

\bibitem{Polvara2018}
R.~Polvara, M.~Patacchiola, S.~Sharma, J.~Wan, A.~Manning, R.~Sutton, and
  A.~Cangelosi, ``Toward end-to-end control for uav autonomous landing via deep
  reinforcement learning,'' in \emph{2018 International Conference on Unmanned
  Aircraft Systems (ICUAS)}, 2018, pp. 115--123.

\bibitem{Polvara2019}
R.~Polvara, S.~Sharma, J.~Wan, A.~Manning, and R.~Sutton, ``Autonomous
  vehicular landings on the deck of an unmanned surface vehicle using deep
  reinforcement learning,'' \emph{Robotica}, vol.~37, no.~11, p. 1867–1882,
  2019.

\bibitem{Rodriguez-Ramos2018}
A.~Rodriguez-Ramos, C.~Sampedro, H.~Bavle, I.~G. Moreno, and P.~Campoy, ``A
  deep reinforcement learning technique for vision-based autonomous multirotor
  landing on a moving platform,'' in \emph{2018 IEEE/RSJ International
  Conference on Intelligent Robots and Systems (IROS)}, 2018, pp. 1010--1017.

\bibitem{Lee2018}
S.~Lee, T.~Shim, S.~Kim, J.~Park, K.~Hong, and H.~Bang, ``Vision-based
  autonomous landing of a multi-copter unmanned aerial vehicle using
  reinforcement learning,'' in \emph{2018 International Conference on Unmanned
  Aircraft Systems (ICUAS)}, 2018, pp. 108--114.

\bibitem{Even-Dar2003}
E.~Even-Dar and Y.~Mansour, ``Learning rates for q-learning,'' \emph{Journal of
  Machine Learning Research}, vol.~5, p. 1–25, 2004.

\bibitem{Narvekar2020}
S.~Narvekar, B.~Peng, M.~Leonetti, J.~Sinapov, M.~E. Taylor, and P.~Stone,
  ``Curriculum learning for reinforcement learning domains: A framework and
  survey,'' \emph{Journal of Machine Learning Research}, vol.~21, 2022.

\bibitem{Anderson1994}
C.~W. Anderson and S.~G. Crawford-Hines, ``Multigrid q-learning. technical
  report cs-94-121,'' 1994.

\bibitem{Furrer2016}
F.~Furrer, M.~Burri, M.~Achtelik, and R.~Siegwart, \emph{Robot Operating System
  (ROS): The Complete Reference (Volume 1)}.\hskip 1em plus 0.5em minus
  0.4em\relax Cham: Springer International Publishing, 2016, ch. RotorS---A
  Modular Gazebo MAV Simulator Framework, pp. 595--625.

\bibitem{Sanches-Cuevas2017}
P.~Sanchez-Cuevas, G.~Heredia, and A.~Ollero, ``Characterization of the
  aerodynamic ground effect and its influence in multirotor control,''
  \emph{International Journal of Aerospace Engineering}, vol. 2017, 2017.

\end{thebibliography}
